ImageNet-21K Pretraining for the Masses

ImageNet-1K serves as the primary dataset for pretraining deep learning models for computer vision tasks. ImageNet-21K dataset, which is bigger and more diverse, is used less frequently for pretraining, mainly due to its complexity, low accessibility, and underestimation of its added value. This paper aims to close this gap, and make high-quality efficient pretraining on ImageNet-21K available for everyone. Via a dedicated preprocessing stage, utilization of WordNet hierarchical structure, and a novel training scheme called semantic softmax, we show that various models significantly benefit from ImageNet-21K pretraining on numerous datasets and tasks, including small mobile-oriented models. We also show that we outperform previous ImageNet-21K pretraining schemes for prominent new models like ViT and Mixer. Our proposed pretraining pipeline is efficient, accessible, and leads to SoTA reproducible results, from a publicly available dataset. The training code and pretrained models are available at: https://github.com/Alibaba-MIIL/ImageNet21K

==> Tables/kd_comparisons.tex <==
\begin{table}[hbt!]
\centering
\begin{tabular}{|c|c|c|} 
\hline
Dataset                           & \begin{tabular}[c]{@{}c@{}}Sematic\\Softmax\\Pretrain\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sematic\\Softmax\\+ Semanic KD\\Pretrain\\\end{tabular}  \\ 
\hline\hline
ImageNet1K\textsuperscript{(1)}   & 81.4                                                               & \textbf{82.2}                                                                       \\ 
\hline
iNaturalist\textsuperscript{(1)}  & 72.0                                                               & \textbf{72.7}                                                                       \\ 
\hline
Food 251\textsuperscript{(1) }    & 75.8                                                               & \textbf{76.1}                                                                       \\ 
\hline
CIFAR 100\textsuperscript{(1) }   & 90.4                                                               & \textbf{91.7}                                                                       \\ 
\hline\hline
MS-COCO\textsuperscript{(2)}      & 81.3                                                               & \textbf{82.2}                                                                       \\ 
\hline
Pascal-VOC\textsuperscript{(2)}   & 89.7                                                               & \textbf{89.8}                                                                       \\ 
\hline\hline
Kinetics 200\textsuperscript{(3)} & 83.0                                                               & \textbf{84.4}                                                                       \\
\hline
\end{tabular}
\caption{\textbf{Testing the effect of semantic KD on downstream results.} Dataset types and metrics: (1) - single-label, top-1 Acc.[$\%$] ; (2) - multi-label, mAP [$\%$]; (3) - action recognition, top-1 Acc. [$\%$]. }
\label{table:kd_comparisons}
\end{table}

==> checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{appendix:limitations} in the appendix}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{We don't think our work can have negative societal impact}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the URL, which has reproduction code and instructions for obtaining the dataset}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{appendix:training_details} in the appendix, and the URL for reproduction code}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{appendix:training_details} in the appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See the URL}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the URL}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We are starting from an existing dataset, which have been used extensively in the past, and follow its usage license}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We are starting from an existing dataset, which have been used extensively in the past, and follow its usage license}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

